Bottom quark forward-backward asymmetry at the future electron-positron collider FCC-ee

The Standard Model (SM) prediction for the \PZ-boson pole $b$-quark forward-backward (FB) asymmetry is: $(A_{FB}^{0,b})_{th} = 0.1030 \pm 0.0002$. The LEP electron-positron collider measured instead $A_{FB}^{0,b} = 0.0992 \pm 0.0016$, value which presents the largest discrepancy with any of the SM predictions as of today. All the $A_{FB}^b$ measurements performed at LEP suffered however of an important statistical uncertainty and of different sources of systematic uncertainties. This study shows that the proposed high-luminosity electron-positron collider FCC-ee, collecting orders of magnitude more data at the \PZ-pole than LEP, will significantly reduce the statistical uncertainties on the measurement of $A_{FB}^{0,b}$, thus allowing us to shed further light on this tension.

==> sections/introduction/formatting.tex <==

\vspace*{.5cm}
\hrule
\vspace*{-.2cm}

\section*{Document formatting convention requests}

Please follow this guidance to help the editors incorporate your text in the final report:

\subsection*{Particle symbols}
For particles, please use the \texttt{heppennames2} package (included).

\noindent For example:
\begin{itemize}[nosep]
\item $\PQt\PAQt$ is \verb+$\PQt\PAQt$+ (which also has the local alias \verb+\ttbar+)
\item $\PH\to\PQb\PAQb$ is \verb+$\PH\to\PQb\PAQb$+ (which also has the local alias \verb+\Hbb+)
\end{itemize}
Please feel free to add other useful aliases to the relevant section of \texttt{ECFAreport\_definitions.sty}.

\subsection*{Units}
For units, please use the \texttt{siunitx} package.

\noindent For example:
\begin{itemize}[nosep]
\item \SI{3.1}{\per\atto\barn} is \verb+\SI{3.1}{\per\atto\barn}+
\item \SI{3.45d-4}{\micro\metre} is \verb+\SI{3.45d-4}{\micro\metre}+
\item \SI{13}{\giga\electronvolt} is \verb+\SI{13}{\giga\electronvolt}+
\end{itemize}

\subsection*{References}
Please use the \texttt{cleveref} package via the commands \texttt{\textbackslash cref} command which takes care of Fig. or Figure in an automatic way. Capitalize the c at the beginning of a sentence etc \texttt{\textbackslash Cref}

\subsection*{Paper References}
Please use the \texttt{\textbackslash cite} commands, and \texttt{\textbackslash biber},
For example \verb+\cite{deBlas:2024bmz}+ \cite{deBlas:2024bmz}.
For example \verb+\cite{ALEPH:2005ab}+ \cite{ALEPH:2005ab}.


\vspace*{.3cm}
\hrule



==> sections/introduction/introduction_old.tex <==
\section{Introduction}

Main text starts here...

Suggest commenting out the table of contents if the document is a short 2-page summary note.  


==> sections/mainbody/theo.tex <==
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Theoretical Framework}\label{Theoretical-Framework}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%


The forward-backward asymmetry in the process $e^+ e^- \to Z \to b \bar b$ is
induced by the parity-violating nature of the neutral weak
current, which manifests itself as an odd contribution to the term linear in $\cos\theta$
in the corresponding differential cross-section~\cite{Tenchini:2008zz}, 

%----------------------------------
\begin{equation}
\frac{d\sigma}{d\cos {\theta}} = 
\sigma^{\text{tot}}_{b \bar {b}}
\left[\frac{3}{8}(1 + \cos^{2} \theta)+ 
A_{FB}^{b} \cos {\theta} \right]\,,
\label{eq:fit_to_cos}
\end{equation}
%----------------------------------

where $\theta$ is defined as the polar scattering angle between the outgoing 
quark and the incoming electron flight directions. The coefficient of the linear term in $\cos\theta$, in the SM and for pure $Z$-boson exchange is related 
at leading order (LO) to the vector and axial-vector couplings 
of the $Z$-boson to the electron and $b$-quark~\cite{ALEPH:2005ab}. 
Due to the values of the $Z$-boson couplings to fermions, both the $A_{FB}^{f \bar f}$ 
asymmetry and its sensitivity to the $\sin^2 \theta_W$ are larger in the 
$Z \to q \bar{q}$ channels with respect to the leptonic ones. 
Hence, the heavy flavor $A_{FB}^{b \bar b}$ and $A_{FB}^{c \bar c}$ asymmetry 
measurements are of particular interest.
Due to large $Z$-boson coupling to the down-type quark (i.e. $Z\to b \bar b$), and 
because of properly identifying $b$-quark through to the secondary vertex, 
the bottom quark $A_{FB}^{0,b}$ 
is the most accurately measured at LEP with 
a 1.6\% precision~\cite{ALEPH:2005ab,TLEPDesignStudyWorkingGroup:2013myl}.

The asymmetry at the $e^+ e^- \to Z \to b \bar b$ events is diluted by the effect 
of mixing in the $B^0 - \bar{B}^0$ system. 
Such kind of effect arises from box diagrams involving mainly virtual top 
quarks~\cite{ALEPH:2005ab,dEnterria:2020cgt}. The average mixing parameter 
denoted by $\chi$ represents the probability that a produced $b$-hadron decays 
likewise its antiparticle. It relates the observed $b$-quark
asymmetry $A_{FB}^{b, \text{obs}}$ to the theoretical 
asymmetry $A_{FB}^{b}$~\footnote{$A_{FB}^{b}$ refers to the general definition 
of the $b$-quark FB asymmetry, while the notation $A_{FB}^{0,b}$ is used if that asymmetry is 
evaluated at the Z-pole.} through the following equation:


%----------------------------------
\begin{equation}
A_{FB}^{b, \text{obs}} = (1 - 2 \chi ) A_{FB}^{b} \,.
\label{eq:AFB-os-th}
\end{equation}
%----------------------------------

